Multi-Hypothesis Visual-Inertial Flow

Estimating the correspondences between pixels in sequences of images is a critical first step for a myriad of tasks including vision-aided navigation (e.g., visual odometry (VO), visual-inertial odometry (VIO), and visual simultaneous localization and mapping (VSLAM)) and anomaly detection. We introduce a new unsupervised deep neural network architecture called the Visual Inertial Flow (VIFlow) network and demonstrate image correspondence and optical flow estimation by an unsupervised multi-hypothesis deep neural network receiving grayscale imagery and extra-visual inertial measurements. VIFlow learns to combine heterogeneous sensor streams and sample from an unknown, un-parametrized noise distribution to generate several (4 or 8 in this work) probable hypotheses on the pixel-level correspondence mappings between a source image and a target image . We quantitatively benchmark VIFlow against several leading vision-only dense correspondence and flow methods and show a substantial decrease in runtime and increase in efficiency compared to all methods with similar performance to state-of-the-art (SOA) dense correspondence matching approaches. We also present qualitative results showing how VIFlow can be used for detecting anomalous independent motion.

==> tex_figures/euroc_sample_results.tex <==
\begin{figure*}[th]
	\begin{minipage}{.3\textwidth}
		\begin{subfigure}{0.33\linewidth}
			\begin{subfigure}{\linewidth}
				\includegraphics[width=\textwidth]{figures/Euroc_Sample_01_source.eps}
				\caption{Source}
	  		\end{subfigure}%
			\begin{subfigure}{\linewidth}
				\includegraphics[width=\textwidth]{figures/Euroc_Sample_01_target.eps}
				\caption{Target}
	  		\end{subfigure}%
			\begin{subfigure}{\linewidth}
				\includegraphics[width=\textwidth]{figures/Euroc_Sample_01_bi.eps}
				\caption{IDE}
	 	 	\end{subfigure}%	  	
	 	 \end{subfigure}%	  
	 	 	
		\begin{subfigure}{\linewidth}
    			\begin{subfigure}{0.5\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/Euroc_Sample_01_de_source.eps}
  	   			%\caption{IDE src. pts.}
  	   			%\hfill
  	 		\end{subfigure}% 
    			\begin{subfigure}{0.5\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/Euroc_Sample_01_de_target.eps}
  	   			%\caption{IDE tgt. pts.}
  	   			%\hfill
  	 		\end{subfigure}%   	 		
  	 		\caption{IDE key points}
	 	 \end{subfigure}%	  		 		  	
	 \end{minipage}
	\hfill
	\begin{minipage}{.3\textwidth}
		\begin{subfigure}{0.33\linewidth}
			\begin{subfigure}{\linewidth}
				\includegraphics[width=\textwidth]{figures/Euroc_Sample_03_source.eps}
				\caption{Source}
	  		\end{subfigure}%
			\begin{subfigure}{\linewidth}
				\includegraphics[width=\textwidth]{figures/Euroc_Sample_03_target.eps}
				\caption{Target}
	  		\end{subfigure}%
			\begin{subfigure}{\linewidth}
				\includegraphics[width=\textwidth]{figures/Euroc_Sample_03_bi.eps}
				\caption{IDE}
	 	 	\end{subfigure}%	  	
	 	 \end{subfigure}%	  
	 	 	
		\begin{subfigure}{\linewidth}
    			\begin{subfigure}{0.5\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/Euroc_Sample_03_de_source.eps}
	  			%\caption{IDE src. pts.}
  	   			%\hfill
  	 		\end{subfigure}% 
    			\begin{subfigure}{0.5\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/Euroc_Sample_03_de_target.eps}
  	   			%\caption{IDE tgt. pts.}  	   			
  	   			%\hfill
  	 		\end{subfigure}%   	 
			\caption{IDE key points}
		
	 	 \end{subfigure}%	  		 		  	
	 \end{minipage}	 
	 \hfill
	\begin{minipage}{.3\textwidth}
		\begin{subfigure}{0.33\linewidth}
			\begin{subfigure}{\linewidth}
				\includegraphics[width=\textwidth]{figures/Euroc_Sample_04_source.eps}
				\caption{Source}
	  		\end{subfigure}%
			\begin{subfigure}{\linewidth}
				\includegraphics[width=\textwidth]{figures/Euroc_Sample_04_target.eps}
				\caption{Target}
	  		\end{subfigure}%
			\begin{subfigure}{\linewidth}
				\includegraphics[width=\textwidth]{figures/Euroc_Sample_04_bi.eps}
				\caption{IDE}
	 	 	\end{subfigure}%	  	
	 	 \end{subfigure}%	  
	 	 	
		\begin{subfigure}{\linewidth}
    			\begin{subfigure}{0.5\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/Euroc_Sample_04_de_source.eps}
	  			%\caption{IDE src. pts.}  	   			
  	   			%\hfill
  	 		\end{subfigure}% 
    			\begin{subfigure}{0.5\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/Euroc_Sample_04_de_target.eps}
	  			%\caption{IDE tgt. pts.}  	   		
  	   			%\hfill
  	 		\end{subfigure}%   	
  	 		\caption{IDE key points}  	 		 		
	 	 \end{subfigure}%	  		 		  	
	 \end{minipage}	 	 
	\caption{Sample EuRoc correspondence results. Note that only every only keypoint (horizontally and vertically) is shown and the actual, unaltered output is fully dense. }		
	\label{euroc_sample_results} 
\end{figure*}  

==> tex_figures/euroc_sample_results_small.tex <==
\begin{figure}[th]
	\begin{minipage}{.4\textwidth}
		\begin{subfigure}{\linewidth}
    			\begin{subfigure}{0.24\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/Euroc_Sample_01_de_source.eps}
  	   			%\caption{IDE src. pts.}
  	   			%\hfill
  	 		\end{subfigure}% 
    			\begin{subfigure}{0.24\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/Euroc_Sample_01_de_target.eps}
  	   			%\caption{IDE tgt. pts.}
  	   			%\hfill
  	 		\end{subfigure} \hfill% %\hspace{0.02\linewidth}% 
    			\begin{subfigure}{0.24\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/Euroc_Sample_02_de_source.eps}
  	   			%\caption{IDE tgt. pts.}
  	   			%\hfill
  	 		\end{subfigure}%    	 
    			\begin{subfigure}{0.24\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/Euroc_Sample_02_de_target.eps}
  	   			%\caption{IDE tgt. pts.}
  	   			%\hfill
  	 		\end{subfigure}%     	 						
	 	 \end{subfigure}%	  		
	 \end{minipage}
	\begin{minipage}{.4\textwidth}
		\begin{subfigure}{\linewidth}
    			\begin{subfigure}{0.24\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/KITTI_Sample_01_de_source.eps}
  	   			%\caption{IDE src. pts.}
  	   			%\hfill
  	 		\end{subfigure}% 
    			\begin{subfigure}{0.24\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/KITTI_Sample_01_de_target.eps}
  	   			%\caption{IDE tgt. pts.}
  	   			%\hfill
  	 		\end{subfigure} \hfill% %\hspace{0.02\linewidth}% 
    			\begin{subfigure}{0.24\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/KITTI_Sample_02_de_source.eps}
  	   			%\caption{IDE tgt. pts.}
  	   			%\hfill
  	 		\end{subfigure}%    	 
    			\begin{subfigure}{0.24\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/KITTI_Sample_02_de_target.eps}
  	   			%\caption{IDE tgt. pts.}
  	   			%\hfill
  	 		\end{subfigure}%     	 						
	 	 \end{subfigure}%	  		
	 \end{minipage}	 
	\caption{Sample EuRoc (top row) and KITTI (bottom row) correspondence results. Note that only every only keypoint (horizontally and vertically) is shown and the actual, unaltered output is fully dense. }		
\end{figure}  
%\begin{figure}[th]
%\centering
%\begin{tabular}[c]{cc}
%	\begin{subfigure}[c]{0.4\textwidth}
%		\includegraphics[width=\linewidth]{figures/Euroc_Sample_01_de_source.eps}
%	\end{subfigure}
%	\begin{subfigure}[c]{0.4\textwidth}
%		\includegraphics[width=\linewidth]{figures/Euroc_Sample_01_de_target.eps}
%	\end{subfigure}
%\end{tabular} 	
%\end{figure}  


==> tex_figures/kitti_sample_results.tex <==
\begin{figure*}[th]
	\begin{minipage}{.3\textwidth}
		\begin{subfigure}{0.33\linewidth}
			\begin{subfigure}{\linewidth}
				\includegraphics[width=\textwidth]{figures/KITTI_Sample_06_source.eps}
				\caption{Source}
	  		\end{subfigure}%
			\begin{subfigure}{\linewidth}
				\includegraphics[width=\textwidth]{figures/KITTI_Sample_06_target.eps}
				\caption{Target}
	  		\end{subfigure}%
			\begin{subfigure}{\linewidth}
				\includegraphics[width=\textwidth]{figures/KITTI_Sample_06_bi.eps}
				\caption{IDE}
	 	 	\end{subfigure}%	  	
	 	 \end{subfigure}%	  
	 	 	
		\begin{subfigure}{\linewidth}
    			\begin{subfigure}{0.5\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/KITTI_Sample_06_de_source.eps}
  	   			%\caption{IDE src. pts.}
  	   			%\hfill
  	 		\end{subfigure}% 
    			\begin{subfigure}{0.5\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/KITTI_Sample_06_de_target.eps}
  	   			%\caption{IDE tgt. pts.}
  	   			%\hfill
  	 		\end{subfigure}%   	 		
  	 		\caption{IDE key points}
	 	 \end{subfigure}%	  		 		  	
	 \end{minipage}
	\hfill
	\begin{minipage}{.3\textwidth}
		\begin{subfigure}{0.33\linewidth}
			\begin{subfigure}{\linewidth}
				\includegraphics[width=\textwidth]{figures/KITTI_Sample_02_source.eps}
				\caption{Source}
	  		\end{subfigure}%
			\begin{subfigure}{\linewidth}
				\includegraphics[width=\textwidth]{figures/KITTI_Sample_02_target.eps}
				\caption{Target}
	  		\end{subfigure}%
			\begin{subfigure}{\linewidth}
				\includegraphics[width=\textwidth]{figures/KITTI_Sample_02_bi.eps}
				\caption{IDE}
	 	 	\end{subfigure}%	  	
	 	 \end{subfigure}%	  
	 	 	
		\begin{subfigure}{\linewidth}
    			\begin{subfigure}{0.5\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/KITTI_Sample_02_de_source.eps}
	  			%\caption{IDE src. pts.}
  	   			%\hfill
  	 		\end{subfigure}% 
    			\begin{subfigure}{0.5\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/KITTI_Sample_02_de_target.eps}
  	   			%\caption{IDE tgt. pts.}  	   			
  	   			%\hfill
  	 		\end{subfigure}%   	 
			\caption{IDE key points}
		
	 	 \end{subfigure}%	  		 		  	
	 \end{minipage}	 
	 \hfill
	\begin{minipage}{.3\textwidth}
		\begin{subfigure}{0.33\linewidth}
			\begin{subfigure}{\linewidth}
				\includegraphics[width=\textwidth]{figures/KITTI_Sample_04_source.eps}
				\caption{Source}
	  		\end{subfigure}%
			\begin{subfigure}{\linewidth}
				\includegraphics[width=\textwidth]{figures/KITTI_Sample_04_target.eps}
				\caption{Target}
	  		\end{subfigure}%
			\begin{subfigure}{\linewidth}
				\includegraphics[width=\textwidth]{figures/KITTI_Sample_04_bi.eps}
				\caption{IDE}
	 	 	\end{subfigure}%	  	
	 	 \end{subfigure}%	  
	 	 	
		\begin{subfigure}{\linewidth}
    			\begin{subfigure}{0.5\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/KITTI_Sample_04_de_source.eps}
	  			%\caption{IDE src. pts.}  	   			
  	   			%\hfill
  	 		\end{subfigure}% 
    			\begin{subfigure}{0.5\linewidth}
  	   			\includegraphics[width=\linewidth]{figures/KITTI_Sample_04_de_target.eps}
	  			%\caption{IDE tgt. pts.}  	   		
  	   			%\hfill
  	 		\end{subfigure}%   	
  	 		\caption{IDE key points}  	 		 		
	 	 \end{subfigure}%	  		 		  	
	 \end{minipage}	 	 
	\caption{Sample KITTI correspondence results. Note that only every only keypoint (horizontally and vertically) is shown and the actual, unaltered output is fully dense.}		 
\end{figure*}  
